GPU Under Pressure: Estimating Application's Stress via Telemetry and Performance Counters

Graphics Processing Units (GPUs) are specialized accelerators in data centers and high-performance computing (HPC) systems, enabling the fast execution of compute-intensive applications, such as Convolutional Neural Networks (CNNs). However, sustained workloads can impose significant stress on GPU components, raising reliability concerns due to potential faults that corrupt the intermediate application computations, leading to incorrect results. Estimating the stress induced by an application is thus crucial to predict reliability (with\,special\,emphasis\,on\,aging\,effects). In this work, we combine online telemetry parameters and hardware performance counters to assess GPU stress induced by different applications. The experimental results indicate the stress induced by a parallel workload can be estimated by combining telemetry data and Performance Counters that reveal the efficiency in the resource usage of the target workload. For this purpose the selected performance counters focus on measuring the i) throughput, ii) amount of issued instructions and iii) stall events.

==> tables/PC_description.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{l|l|l|l}
\hline
Group                          & Metric name                                                 & Performance counter                                                                                                    & Description                                                                                                                                                                                            \\ \hline
\multirow{7}{*}{Throughput}    & sm__inst_executed_pipe_alu                                  & Executed Aritmetic Logic Units                                                                                         & \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Counters that are used to describe\\ operational throughput in terms of \\ executed operations.\end{tabular}}                                               \\ \cline{2-3}
                               & sm__inst_executed_pipe_fp16                                 & \begin{tabular}[c]{@{}l@{}}Executed operations between \\ Floating Point 16 bits\end{tabular}                          &                                                                                                                                                                                                        \\ \cline{2-3}
                               & sm__inst_executed_pipe_fp64_op_fp64                         & \begin{tabular}[c]{@{}l@{}}Executed operations between \\ Floating Point 64 bits\end{tabular}                          &                                                                                                                                                                                                        \\ \cline{2-3}
                               & sm__inst_executed_pipe_tensor_op_dmma                       & \begin{tabular}[c]{@{}l@{}}Executed Dot Product operations\\ from Tensor Core Unit\end{tabular}                        &                                                                                                                                                                                                        \\ \cline{2-3}
                               & sm__inst_executed_pipe_tensor_op_hmma                       & \begin{tabular}[c]{@{}l@{}}Executed operations between \\ Floating Point 16 bits from Tensor\\ Core Units\end{tabular} &                                                                                                                                                                                                        \\ \cline{2-3}
                               & sm__inst_executed_pipe_tensor_op_imma                       & \begin{tabular}[c]{@{}l@{}}Executed operations between \\ Integers from Tensor Core Units\end{tabular}                 &                                                                                                                                                                                                        \\ \cline{2-3}
                               & sm__inst_executed_pipe_xu                                   & \begin{tabular}[c]{@{}l@{}}Executed special operations\\ (e.g., sin, cos, log)\end{tabular}                            &                                                                                                                                                                                                        \\ \hline
Issued instructions            & smsp__inst_issued                                           & \begin{tabular}[c]{@{}l@{}}Number of issued instruction \\ per SM SubPartition\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}Counters that consider all the \\ possible SASS instructions \\ (e.g., LOAD, ADD, FETCH) that\\ have been issued for each warp.\end{tabular}                                \\ \hline
\multirow{12}{*}{Stall events} & smsp__warp_issue_stalled_imc_miss_per_warp_active           & Memory stall                                                                                                           & \begin{tabular}[c]{@{}l@{}}Stall due to constant memory \\ dependency.\end{tabular}                                                                                                                    \\ \cline{2-4} 
                               & smsp__warp_issue_stalled_long_scoreboard_per_warp_active    & Memory stall                                                                                                           & \begin{tabular}[c]{@{}l@{}}Stall due to the application waiting\\ for data to be read.\end{tabular}                                                                                                    \\ \cline{2-4} 
                               & smsp__warp_issue_stalled_wait_per_warp_active               & Scheduler stall                                                                                                        & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Stall due to divergences or \\ kernels syncronization issues \\ (e.g., divergences or barriers).\end{tabular}}                                              \\ \cline{2-3}
                               & smsp__warp_issue_stalled_short_scoreboard_per_warp_active   & Scheduler stall                                                                                                        &                                                                                                                                                                                                        \\ \cline{2-3}
                               & smsp__warp_issue_stalled_sleeping_per_warp_active           & Scheduler stall                                                                                                        &                                                                                                                                                                                                        \\ \cline{2-3}
                               & smsp__warp_issue_stalled_barrier_per_warp_active            & Scheduler stall                                                                                                        &                                                                                                                                                                                                        \\ \cline{2-3}
                               & smsp__warp_issue_stalled_membar_per_warp_active             & Scheduler stall                                                                                                        &                                                                                                                                                                                                        \\ \cline{2-3}
                               & smsp__warp_issue_stalled_tex_throttle_per_warp_active       & Scheduler stall                                                                                                        &                                                                                                                                                                                                        \\ \cline{2-4} 
                               & smsp__warp_issue_stalled_mio_throttle_per_warp_active       & Throttle stall                                                                                                         & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Stall due to the throttle mechanism\\ activated for not enough resources\\ available (e.g., in terms of \\ computational units, memory slots)\end{tabular}} \\ \cline{2-3}
                               & smsp__warp_issue_stalled_math_pipe_throttle_per_warp_active & Throttle stall                                                                                                         &                                                                                                                                                                                                        \\ \cline{2-3}
                               & smsp__warp_issue_stalled_lg_throttle_per_warp_active        & Throttle stall                                                                                                         &                                                                                                                                                                                                        \\ \cline{2-3}
                               & smsp__warp_issue_stalled_drain_per_warp_active              & Throttle stall                                                                                                         &                                                                                                                                                                                                        \\ \hline
\end{tabular}
\end{table}

==> tables/experimental_setup.tex <==
\begin{table}[]
\caption{Experimental Setup outline}
\begin{tabular}{cccc}
\hline
\textit{\textbf{\begin{tabular}[c]{@{}c@{}}Application\\ name\end{tabular}}} & \textit{\textbf{Domain}}                                         & \textit{\textbf{Suite}} & \textit{\textbf{\begin{tabular}[c]{@{}c@{}}Simulation\\ Parameters\end{tabular}}} \\ \hline
\textbf{GPU-burn}                                                            & \begin{tabular}[c]{@{}c@{}}Matrix \\ Multiplication\end{tabular} & GPU-burn                & \begin{tabular}[c]{@{}c@{}}Time = 5 mins\\ Mem. occ. = 50\%\end{tabular}          \\ \hline
\textbf{LeNet5}                                                              & CNN                                                              & Torchvision             & \begin{tabular}[c]{@{}c@{}}Iterations= 100\\ Batch size = 10000\end{tabular}      \\ \hline
\textbf{MnasNet}                                                             & CNN                                                              & Torchvision             & \begin{tabular}[c]{@{}c@{}}Iterations= 100\\ Batch size = 10000\end{tabular}      \\ \hline
\textbf{MobileNetV2}                                                         & CNN                                                              & Torchvision             & \begin{tabular}[c]{@{}c@{}}Iterations = 100\\ Batch size = 2048\end{tabular}      \\ \hline
\textbf{Resnet18}                                                            & CNN                                                              & Torchvision             & \begin{tabular}[c]{@{}c@{}}Iterations = 100\\ Batch size = 4096\end{tabular}      \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Back \\ Propagation\end{tabular}}         & \begin{tabular}[c]{@{}c@{}}Machine \\ learning\end{tabular}      & Rodinia                 & Iterations = 45000                                                                \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Gaussian\\ Elimination\end{tabular}}      & \begin{tabular}[c]{@{}c@{}}Linear \\ algebra\end{tabular}        & Rodinia                 & Iterations = 1500                                                                 \\ \hline
\textbf{Hotspot}                                                             & \begin{tabular}[c]{@{}c@{}}Structured \\ Grid\end{tabular}       & Rodinia                 & Iterations = 25000                                                                \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Needleman\\ Wunsch\end{tabular}}          & \begin{tabular}[c]{@{}c@{}}Linear \\ algebra\end{tabular}        & Rodinia                 & Iterations = 1500                                                                 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Stream\\ Cluster\end{tabular}}            & \begin{tabular}[c]{@{}c@{}}Machine \\ learning\end{tabular}      & Rodinia                 & Iterations = 25000                                                                \\ \hline
\end{tabular}
\label{tab:apps}
\end{table}

==> tables/metrics.tex <==
\begin{table}[]
\caption{Derived metric from the Performance Counters sampling.}
\begin{tabular}{c|c|c}
\hline
\textit{\textbf{\begin{tabular}[c]{@{}c@{}}Metric \\ name\end{tabular}}} & \textit{\textbf{Formula}}                               & \textit{\textbf{Description}}                                                                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}SM \\ busy\\ rate\end{tabular}                & $\frac{\frac{\#Arithmetic\_instructions}{Warp\_size}}{SM\_busy\_rate_{Pk}} \times 100$ & \begin{tabular}[c]{@{}c@{}}Number of arithmetic \\ instructions executed \\ per cycle per SM \\ w.r.t. its HW peak.\end{tabular}                                                                              \\ \hline
AEI                                                                      & $\frac{\frac{\#Executed\_instructions}{\# Active\_cycles}}{AEI_{Pk}} \times 100$    & \begin{tabular}[c]{@{}c@{}}Number of instructions \\ that were requested and \\ executed during the \\ active cycles per SM \\ w.r.t. its HW peak.\end{tabular}          \\ \hline
AII                                                                      & $\frac{\frac{\#Issued\_instructions}{\# Active\_cycles}}{AII_{Pk}} \times 100$      & \begin{tabular}[c]{@{}c@{}}Number of instructions\\  requested but not \\ executed during the \\ active cycles per SM \\ w.r.t. its HW peak.\end{tabular}       \\ \hline
$S_{act}$                                                                & $ \frac{S_{throt} + S_{cont} + S_{mem}}{S_{TOT}}\times 100 $                      & \begin{tabular}[c]{@{}c@{}}Percentage of stalls \\ due to throttle,\\ scheduling policy and \\ available memory \\ w.r.t. all stall reasons.\end{tabular}
\end{tabular}
\label{tab:metrics}
\end{table}

==> tables/results.tex <==
\begin{table*}[]
\caption{The table summarizes the behavior of each application in terms of architectural activity and system-level telemetry. In this table, \textit{Parameters} column summarizes workload settings: Mem is the GPU memory usage, Batch is the the neural network batch size, and It is the the number of iterations.}
\begin{tabular}{ccc|cccc|cccc}
\hline
\textit{\textbf{Application}}                                            & \textit{\textbf{Domain}}                                        & \textit{\textbf{Parameters}}                                        & \textit{\textbf{\begin{tabular}[c]{@{}c@{}}SM busy\\ rate [\%]\end{tabular}}} & \textit{\textbf{AEI [\%]}} & \textit{\textbf{AII [\%]}} & \textit{\textbf{S$_{act}$ [\%]}} & \textit{\textbf{T$_{\infty}$ [°C]}} & \textit{\textbf{t$_r$ [s]}} & \textit{\textbf{Pow [kJ/min]}} & \textit{\textbf{CF [GHz]}} \\ \hline
\textbf{GPU-burn \cite{defour2013gpuburn}}                                                        & \begin{tabular}[c]{@{}c@{}}Matrix\\ Multiplication\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time = 5 mins\\ Mem. = 50\%\end{tabular} & 74.82                                                                         & 2.99                       & 74.81                      & 9.162                           & 64.97                       & 115                         & 7.12                           & 1.36                       \\ \hline
\textbf{LeNet5 \cite{marcel2010torchvision}}                                                          & CNN                                                             & \begin{tabular}[c]{@{}c@{}}It= 100\\ Batch = 10000\end{tabular}     & 55.69                                                                         & 1.86                       & 21.21                      & 49.71                           & 59.5                        & 110                         & 5.44                           & 1.98                       \\
\textbf{MnasNet \cite{marcel2010torchvision}}                                                         & CNN                                                             & \begin{tabular}[c]{@{}c@{}}It= 100\\ Batch = 10000\end{tabular}     & 45.74                                                                         & 1.69                       & 24.69                      & 50.17                           & 63.19                       & 150                         & 6.00                           & 1.79                       \\
\textbf{MobileNetV2 \cite{marcel2010torchvision}}                                                     & CNN                                                             & \begin{tabular}[c]{@{}c@{}}It = 100\\ Batch = 2048\end{tabular}     & 46.49                                                                         & 1.53                       & 25.46                      & 49.96                           & 61.72                       & 140                         & 5.80                           & 1.69                       \\
\textbf{ResNet18 \cite{marcel2010torchvision}}                                                        & CNN                                                             & \begin{tabular}[c]{@{}c@{}}It = 100\\ Batch = 4096\end{tabular}     & 59.04                                                                         & 2.19                       & 24.38                      & 51.74                           & 62.03                       & 145                         & 5.90                           & 1.68                       \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Back \\ Propagation \cite{che2009rodinia}\end{tabular}}     & \begin{tabular}[c]{@{}c@{}}Machine\\ learning\end{tabular}      & It = 45000                                                          & 79.61                                                                         & 2.08                       & 16.30                      & 22.34                           & 54.53                       & 115                         & 5.03                           & 2.03                       \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Elimination \cite{che2009rodinia}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Linear\\ algebra\end{tabular}        & It = 1500                                                           & 11.21                                                                         & 0.41                       & 10.03                      & 42.99                           & 54.05                       & 105                         & 4.94                           & 2.03                       \\ \hline
\textbf{Hostspot \cite{che2009rodinia}}                                                        & \begin{tabular}[c]{@{}c@{}}Structured \\ grid\end{tabular}      & It = 25000                                                          & 88.38                                                                         & 0.35                       & 9.00                       & 24.5                           & 55.45                        & 125                         & 5.42                           & 2.01                       \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Needleman\\ Wunsch \cite{che2009rodinia}\end{tabular}}      & \begin{tabular}[c]{@{}c@{}}Linear \\ algebra\end{tabular}       & It = 1500                                                           & 5.84                                                                          & 0.18                       & 3.79                       & 18.17                           & 53.51                       & 105                         & 4.88                           & 2.03                       \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Stream \\ Cluster \cite{che2009rodinia}\end{tabular}}       & \begin{tabular}[c]{@{}c@{}}Machine \\ learning\end{tabular}     & It = 25000                                                          & 3.48                                                                          & 0.11                       & 3.47                       & 40.78                           & 53.87                       & 110                         & 4.82                           & 2.02                        \\ \hline
\end{tabular}
\label{tab:results}
\end{table*}

==> tables/results_pt2.tex <==
\begin{table*}[]
\caption{The table summarizes the behavior of each application in terms of architectural activity and system-level telemetry. \todo{(use the missing spaces on the left and the right, the table is consuming a lot of space. consider only one row per benchmark)} % \todo{Why $E_{min}$? and not $E$ only, is gives the impression you are reporting the minimum energy} 
% In this table, \textit{Parameters} column summarizes workload settings: Mem is the GPU memory usage, Batch is the neural network batch size, and It is the number of iterations. \begin{tabular}[c]{@{}c@{}}$\lambda$\\ $[\times 10^{-9}]$\end{tabular}
}
\centering
\begin{tabular}{cc|ccc|cccc|c}
\hline
\textit{\textbf{Application}}                                                                                         & \textit{\textbf{Domain}}                                        & \textit{\textbf{\begin{tabular}[c]{@{}c@{}}SM busy\\ rate [\%]\end{tabular}}} & \textit{\textbf{AII [\%]}} & \textit{\textbf{S$_{act}$ [\%]}} & \textit{\textbf{T$_{\infty}$ [°C]}} & \textit{\textbf{t$_r$ [s]}} & \multicolumn{1}{c|}{\textit{\textbf{E [kJ/min]}}} & \textit{\textbf{$\Delta$ CF [MHz]}} \\ \hline
\rowcolor[HTML]{FFCCC9} \textbf{GPU-burn \cite{defour2013gpuburn}}                                                    & \begin{tabular}[c]{@{}c@{}}Matrix\\ Multiplication\end{tabular} & 74.82                                                                         & 74.81                      & 9.162                            & 64.97                               & 115                         & 7.12                                                         & 740                                          \\ \hline
\rowcolor[HTML]{FFCE93} \textbf{LeNet5 \cite{marcel2010torchvision}}                                                  & CNN                                                             & 55.69                                                                         & 21.21                      & 49.71                            & 59.5                                & 110                         & 5.44                                                         & 120                                          \\
\rowcolor[HTML]{FFCE93} \textbf{MnasNet \cite{marcel2010torchvision}}                                                 & CNN                                                             & 45.74                                                                         & 24.69                      & 50.17                            & 63.19                               & 150                         & 6.00                                                         & 310                                           \\
\rowcolor[HTML]{FFCE93} \textbf{MobileNetV2 \cite{marcel2010torchvision}}                                             & CNN                                                             & 46.49                                                                         & 25.46                      & 49.96                            & 61.72                               & 140                         & 5.80                                                         & 410                                           \\
\rowcolor[HTML]{FFCE93} \textbf{ResNet18 \cite{marcel2010torchvision}}                                                & CNN                                                             & 59.04                                                                         & 24.38                      & 51.74                            & 62.03                               & 145                         & 5.90                                                         & 420                                          \\ \hline
\rowcolor[HTML]{FFFC9E}\textbf{\begin{tabular}[c]{@{}c@{}} Back \\ Propagation \end{tabular} \cite{che2009rodinia}}    & \begin{tabular}[c]{@{}c@{}}Machine\\ learning\end{tabular}      & 79.61                                                                         & 16.30                      & 22.34                            & 54.53                               & 115                         & 5.03                                                         & 70                                       \\ \hline
\rowcolor[HTML]{FFFC9E}\textbf{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Elimination\end{tabular}  \cite{che2009rodinia}} & \begin{tabular}[c]{@{}c@{}}Linear\\ algebra\end{tabular}        & 11.21                                                                         & 10.03                      & 42.99                            & 54.05                               & 105                         & 4.94                                                         & 70                                           \\ \hline
\rowcolor[HTML]{FFFC9E} \textbf{Hostspot \cite{che2009rodinia}}                                                       & \begin{tabular}[c]{@{}c@{}}Structured \\ grid\end{tabular}      & 88.38                                                                         & 9.00                       & 24.5                             & 55.45                               & 125                         & 5.42                                                         & 90                                         \\ \hline
\rowcolor[HTML]{FFFC9E}\textbf{\begin{tabular}[c]{@{}c@{}}Needleman\\ Wunsch \end{tabular} \cite{che2009rodinia}}    & \begin{tabular}[c]{@{}c@{}}Linear \\ algebra\end{tabular}       & 5.84                                                                          & 3.79                       & 18.17                            & 53.51                               & 105                         & 4.88                                                         & 70                                              \\ \hline
\rowcolor[HTML]{FFFC9E}\textbf{\begin{tabular}[c]{@{}c@{}}Stream \\ Cluster  \end{tabular}\cite{che2009rodinia}}      & \begin{tabular}[c]{@{}c@{}}Machine \\ learning\end{tabular}     & 3.48                                                                          & 3.47                       & 40.78                            & 53.87                               & 110                         & 4.82                                                         & 90                                             \\ \hline
\end{tabular}
\vspace{-5mm}
\label{tab:results_pt2}
\end{table*}

